The LX-sigma Relation for Galaxies and Clusters of Galaxies

We demonstrate that individual elliptical galaxies and clusters of galaxies form a continuous X-ray luminosity---velocity dispersion (LX-sigma) relation. Our samples of 280 clusters and 57 galaxies have LX ~ sigma^4.4 and LX ~ sigma^10, respectively. This unified LX - sigma relation spans 8 orders of magnitude in LX and is fully consistent with the observed and theoretical luminosity---temperature scaling laws. Our results support the notion that galaxies and clusters of galaxies are the luminous tracers of similar dark matter halos.

==> DATAREADME <==
Contents of this directory:

systemcat---280 objects---catalog of clusters and groups
galaxycat----84 objects---catalog of galaxies

Format of files: whitespace-delimited ASCII text

All cluster X-ray data is from Xue \& Wu (2000) and Wu, Xue, \& Fang
(1999) unless otherwise noted.

All galaxy velocity dispersions are from Faber et al. (1989).

Column		Explanation
------------------------------------------------------
 1		Object name conforming to NED standard
 2-4		RA (J2000)
 5-7		DEC (J2000)
 8		redshift
 9		log velocity dispersion
10		error
11		log bolometric X-ray luminosity (H_0 = 50 km / s / Mpc)
12		error
13		Other identifications / Comments

Key to Comments
------------------------------
H		X-ray luminosity is from Helsdon & Ponman (2000; HP00)
R		X-ray luminosity is from Mahdavi \etal (2000); velocity
		dispersion is from ongoing survey described in
		Mahdavi etal (1999; M99).
HR		Luminosity is from HP00; velocity dispersion is from M99
F		X-ray luminosity is from Eskridge, Fabbiano, & Kim (1995)
B		X-ray luminosity is from Beuing et al. (1999)
AGN		Galaxy contains an active galactic nucleus (rejected)
GR		Galaxy X-ray emission is continuous with larger group or
		cluster emission (rejected)


